Security Vulnerability Detection with Multitask Self-Instructed Fine-Tuning of Large Language Models

Software security vulnerabilities allow attackers to perform malicious activities to disrupt software operations. Recent Transformer-based language models have significantly advanced vulnerability detection, surpassing the capabilities of static analysis based deep learning models. However, language models trained solely on code tokens do not capture either the explanation of vulnerability type or the data flow structure information of code, both of which are crucial for vulnerability detection. We propose a novel technique that integrates a multitask sequence-to-sequence LLM with pro-gram control flow graphs encoded as a graph neural network to achieve sequence-to-classification vulnerability detection. We introduce MSIVD, multitask self-instructed fine-tuning for vulnerability detection, inspired by chain-of-thought prompting and LLM self-instruction. Our experiments demonstrate that MSIVD achieves superior performance, outperforming the highest LLM-based vulnerability detector baseline (LineVul), with a F1 score of 0.92 on the BigVul dataset, and 0.48 on the PreciseBugs dataset. By training LLMs and GNNs simultaneously using a combination of code and explanatory metrics of a vulnerable program, MSIVD represents a promising direction for advancing LLM-based vulnerability detection that generalizes to unseen data. Based on our findings, we further discuss the necessity for new labelled security vulnerability datasets, as recent LLMs have seen or memorized prior datasets' held-out evaluation data.

==> unused.tex <==
The second limitation is that the size of the training dataset constrains the performance of these models

However, these models overlook documentation details about vulnerabilities, such as their vulnerability types, explanations on how certain data flows lead to vulnerabilities, and how certain vulnerabilities could be exploited.


To the best of our knowledge, prior LM based vulnerability detection techniques evaluate on data released before their pre-trained LM's training data cutoff date~\cite{devign, codexglue, linevul, finetuning_vul}, resulting in training data leakage~\cite{wang2024pandora} and an inability to generalize to newer datasets~\cite{deepdfa, llm_comprehensive}.

no prior work has extensively studied the effects of self-instruct fine-tuning on both vulnerability code and vulnerability explanation. Fine-tuning specifically aims to adapt a pre-trained model to a particular domain, and self-instruct aims to train an LLM on question-answer style data. 

